Application-Aware Twin-in-the-Loop Planning for Federated Split Learning over Wireless Edge Networks

We investigate task-success-oriented resource allocation for federated split learning (FSL) at the wireless edge. In this setting, the server must jointly determine bandwidth, transmit power, split-layer placement, compression level, and terminal participation under per-round deadline, memory, and spectrum constraints. These coupled decisions affect wireless transmission, model training, and task execution, which evolve at different time scales and cannot be efficiently evaluated through repeated real-world trials. To address this challenge, we propose TiLP, a twin-in-the-loop planner that evaluates candidate decisions through a cross-domain digital twin before execution. The twin integrates network, training, and task sub-twins, with each sub-twin calibrated at the time scale of the process it models. Based on this twin, TiLP performs receding-horizon cross-entropy method planning with actor-critic guidance to search over mixed continuous-discrete decisions. Experiments on LIBERO robotic manipulation tasks over a Sionna RT-simulated wireless network show that TiLP improves task success by 9.5 percentage points over the strongest single-axis baseline, while satisfying the per-round deadline and energy budget.

==> section/3_system_model.tex <==
%% =====================================================================
%%  Section 3 : System Model and Problem Formulation
%% =====================================================================
\section{System Model and Problem Formulation}
\label{sec:sys}

\subsection{System Overview}
\label{sec:sys-overview}
\label{sec:sys-taskdt}%% legacy label kept for cross-references

% \begin{figure*}
%     \centering
%     \includegraphics[width=1\linewidth]{results/jsac_dt.pdf}
%     \caption{Enter Caption}
%     \label{fig:placeholder}
% \end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{results/network_twin.pdf}
    \caption{Network sub-twin illustration.}
    \label{fig:placeholder}
\end{figure}

Consider an edge AI system with a base station (BS) and a co-located edge server. The BS serves $N$ terminals, which collaboratively fine-tune a shared foundation model $\Phi$ using their private datasets. The training protocol follows federated split learning: each terminal stores the front part of $\Phi$ on the device, while the edge server stores the remaining part.

The training process proceeds over $T$ rounds, and each round must finish within a deadline. Terminal $n$ is constrained by a transmit power $\bar{\mathrm{P}}$ and an on-device memory $\bar{\mathrm{M}}_n$. In FSL, each scheduled terminal must upload split-layer activations and receive the corresponding gradients. As these payloads can be large, especially when the model is split at a deep layer, lossy payload compression is enabled to reduce transmission time and bandwidth usage. The maximum allowable compression level is denoted by $\bar{\rho}$.

In the $t$-th training round, the BS determines five control variables for each terminal. These variables are the allocated bandwidth $\mathrm{b}_n[t]$, the transmit power $\mathrm{p}_n[t]$, the split-layer index $l_n[t]$, the compression level $\rho_n[t]$, and the scheduling indicator $\alpha_n[t]\in\{0,1\}$. If terminal $n$ uses $l_n[t]$, then the terminal executes all layers up to and including layer $l_n[t]$, while the server executes the remaining layers of $\Phi$. The output of layer $l_n[t]$ is then sent to the server. $\rho_n[t]$ signifies a fraction $1-\rho_n[t]$ of the payload is transmitted. A larger $\rho_n[t]$ reduces the communication load, but it also removes more information from the exchanged activations and gradients. We denote the joint action by $a_n[t]\triangleq\bigl(\mathrm{b}_n[t],\mathrm{p}_n[t],l_n[t],\rho_n[t],\alpha_n[t]\bigr)_{n=1}^{N}$.

Note that the joint action $a[t]$ cannot be tried freely on the real system because, once executed, there is no going back--direct execution may lead to unsafe actions before the task outcome is observed. To address this, we build a cross-domain digital twin (DT) $\widehat{\Omega}[t]$ with three coupled sub-twins. The network sub-twin $\widehat{\Omega}^{N}[t]$ simulates the wireless environment. The training sub-twin $\widehat{\Omega}^{L}[t]$ predicts the one-round loss reduction on a model instance. The task sub-twin $\widehat{\Omega}^{T}[t]$ estimates the task success rate of the current model.

% Consider an edge AI system with a base station (BS) and a co-located edge server. The BS serves $N$ terminals, indexed by $n\in\mathcal{N}\triangleq\{1,\ldots,N\}$. The terminals collaboratively fine-tune a shared foundation model $\Phi$ on their private datasets. The training protocol is federated split learning (FSL): each terminal stores the front part of $\Phi$ on device, while the edge server stores the remaining part.

% Training proceeds over $R$ rounds. Each round must finish within a deadline $\bar{\ell}$. The carrier frequency is $f_c$. The noise power spectral density is $N_0$. Terminal $n$ is constrained by a transmit-power budget $\bar{P}$ and an on-device memory budget $\bar{M}_n$. In FSL, each scheduled terminal must upload split-layer activations and receive the corresponding gradients. These payloads can be large, especially when the model is split at a deep layer. As such, lossy payload compression is enabled to reduce transmission time and bandwidth usage. The maximum allowable compression level is denoted by $\bar{\rho}$.

% In round $t$, the BS determines five control variables for each terminal. These variables are the allocated bandwidth $b_n[t]$, the transmit power $p_n[t]$, the split-layer index $j_n[t]\in\mathcal{K}$, the compression level $\rho_n[t]\in[0,\bar{\rho}]$, and the scheduling indicator $m_n[t]\in\{0,1\}$. Here, $\mathcal{K}$ is the set of candidate terminal-side last layers. If terminal $n$ uses $j_n[t]$, then the terminal executes all layers up to and including layer $j_n[t]$, while the server executes the remaining layers. The output of layer $j_n[t]$ is then sent to the server. Also, $\rho_n[t]$ is the fraction of the activation or gradient payload discarded by compression. Therefore, only a fraction $1-\rho_n[t]$ of the payload is transmitted. A larger $\rho_n[t]$ reduces the communication load, but it also removes more information from the exchanged activations and gradients. We denote the set of scheduled terminals by $\mathcal{S}[t]\triangleq\{n\in\mathcal{N}:m_n[t]=1\}$. We denote the joint action by $a[t]\triangleq\bigl(b_n[t],p_n[t],j_n[t],\rho_n[t],m_n[t]\bigr)_{n=1}^{N}$.

% Note that the joint action $a[t]$ cannot be tried freely on the real system because, once executed, there is no going back--it consumes wireless resources, changes the model through one FSL round, and reveals task performance only after evaluation. 
% Note that the joint action $a[t]$ cannot be tried freely on the real system because, once executed, there is no going back. Direct execution may lead to unsafe robot actions before the controller can observe the task outcome.
% To address this, we build a cross-domain digital twin (DT) $\widehat{\Omega}[t]$ with three coupled sub-twins. The network sub-twin $\widehat{\Omega}^{w}[t]$ simulate the wireless environment and predicts the maximum transmission rates. The training sub-twin $\widehat{\Omega}^{l}[t]$ predicts the one-round loss reduction $\Delta\hat{L}[t]$ on an auxiliary model instance. The task sub-twin $\widehat{\Omega}^{r}[t]$ estimates the task success rate $\hat{A}[t]$ of the current model.

\subsection{Network Sub-Twin}
\label{sec:sys-wireless}



% A bandwidth-power allocation cannot be configured arbitrarily on the real network, since a terminal can miss the round deadline (due to the miscalculation of the maximum data rate) and run an outdated model, risking harm to people or equipment. 
% A bandwidth–power allocation cannot be tried on the real network, since a bad allocation delays the next control packet pass the arm's in-progress motion and turns a scheduling error into a collision, so the network twin must check the allocation against the arm's state before the packet is sent.
% If a bad bandwidth-power allocation is tried on the real network, the terminal misses the round deadline and runs an outdated model, risking harm to people or equipment.
In practice, bandwidth and power allocation on the real network must be carefully configured. If the maximum data rate is miscalculated, a terminal may miss its round deadline and operate with an outdated model, which can lead to risks for people or equipment.
The network sub-twin $\widehat{\Omega}^{N}[t]$ simulates the wireless environment and predicts the maximum transmission rate of each terminal for a bandwidth-power pair $(\mathrm{b}_n[t],\mathrm{p}_n[t])$. Let $G_n$ denote the large-scale channel gain of terminal $n$, modeled by a standard path-loss model~\cite{Wang2025MCOM}, the small-scale fading is represented by $H_n[t]\sim\mathcal{CN}(0,1)$. 
% Let also $X_n[t]$ be the transmit symbol with average power $p_n[t]$. Over bandwidth $b_n[t]$, the receiver noise power is $N_0 b_n[t]$. The signal received by the BS from terminal $n$ is
% \begin{equation}
%   Y_n[t] \,=\, \sqrt{G_n}\,H_n[t]\,X_n[t]+Z_n[t],
%   \label{eq:sys-Y}
% \end{equation}
% where $Z_n[t]\sim\mathcal{CN}(0,N_0 b_n[t])$. 
The transmission rate is
\begin{equation}
  R_n[t] \,=\,\mathrm{b}_n[t]\log_{2}\!\Bigl(1+\frac{G_n\,|H_n[t]|^{2}\,\mathrm{p}_n[t]}{N_0\,\mathrm{b}_n[t]}\Bigr).
  \label{eq:sys-R}
\end{equation}


\subsection{Training Sub-Twin}
\label{sec:sys-fsl}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{results/training_twin.pdf}
    \caption{Training sub-twin illustration.}
    \label{fig:placeholder}
\end{figure}

% A candidate split, compression, and scheduling decision cannot be checked freely through real training, because its effect on convergence is only observed after consuming one FSL round. 
% If a split or compression is tried on the real system and found wrong, the network resources spent are wasted and the round deadline is missed.
% If a bad split or compression is tried on the real system, the model is irreversibly corrupted; the update cannot be rolled back, and later rounds can only partially repair rather than undo the damage.
% Likewise, when an inaccurate split and compression are attempted on the real system, the model becomes irreversibly corrupted. The update cannot be undone, and subsequent rounds are only able to partially repair the resulting damage instead of fully reversing it.
% The training sub-twin $\widehat{\Omega}^{L}[t]$ estimates the one-round loss reduction $\Delta{L}[t]$ produced by a candidate action. It captures the communication pattern of FSL and the resulting parameter updates. In particular, it models how the chosen compression level affects the payload size and the subsequent training quality.

Likewise, when an inaccurate split and compression are attempted on the real system, the model becomes irreversibly affected, which can result in unsafe operation of terminals. The update cannot be undone, and subsequent rounds are only able to partially repair the resulting damage instead of fully reversing it.
The training sub-twin $\widehat{\Omega}^{L}[t]$ estimates the one-round loss reduction produced by the compression ratios, split-layer locations, selected terminals, and terminals' memory budget.

At round $t$, terminal $n$ selects layer $l_n[t]$ to serve as its final local layer. The terminal then trains the model from the input up to this layer. After this, the server is responsible for computing the remaining layers. For each scheduled terminal, the local batch samples are processed through the local layers, which produce the activation at the split layer as follows:
\begin{equation}
  \mathbf{S}_n[t] \,=\, \mathfrak{f}\bigl(\mathbf{X}_n[t];\,\mathbf{W}^\textrm{C}_n[t-1]\bigr),
  \label{eq:sys-Sfwd}
\end{equation}
where $\mathbf{W}^\textrm{C}_n[t-1]$ denotes the trainable parameters on the client (terminal) side and $\mathbf{X}_n[t]$ denotes the local batch samples. The activation is compressed with level $\rho_n[t]$ and uploaded to the server together with the labels. The server then continues the model training on the remaining layers, computes the loss, and obtains the corresponding gradients. The server also updates the server-side trainable parameters, compresses the gradient at the split layer at the same level, and sends the result back to the terminal for local back-propagation.

Let $\mathbf{W}^\textrm{S}[t]$ denote the trainable server-side parameters and $\mathbf{W}[t]$ collect all trainable parameters at round $t$, then the server-side update is
\begin{equation}
  \mathbf{W}^{\textrm{S}}[t] \,=\, \mathbf{W}^\textrm{S}[t-1]-\eta^\textrm{S}\,\mathbf{G}^\textrm{S}[t],
  \label{eq:sys-upd-s}
\end{equation}
and the terminal-side update is
\begin{equation}
  \mathbf{W}^\textrm{C}_n[t] \,=\, \mathbf{W}^\textrm{C}_n[t-1]-\eta^\textrm{C}\,\mathbf{G}^\textrm{C}_n[t],
  \label{eq:sys-upd-c}
\end{equation}
where $\eta^\textrm{S}$ and $\eta^\textrm{C}$ are the learning rates, and $\mathbf{G}^\textrm{S}[t]$ and $\mathbf{G}^\textrm{C}_n[t]$ are the gradients of $\mathfrak{L}^\textrm{S}$ and $\mathfrak{L}^\textrm{C}_n$ with respect to $\mathbf{W}^\textrm{S}$ and $\mathbf{W}^\textrm{C}_n$, respectively.

Denote $|D_n|$ as the sample size of terminal $n$ and $D$ as the total number of samples.
Let $f$ denote the average loss over a batch. The server-side loss is observed at the server, which sees only the received activation:
\begin{equation}
  \mathfrak{L}^\textrm{S} \,=\, f\bigl(\mathbf{S}_n[t],\mathbf{W}^\textrm{S}[t-1]\bigr).
  \label{eq:sys-loss-s}
\end{equation}
The client-side loss is observed at terminal $n$, which sees the full forward path from $\mathbf{X}_n[t]$:
\begin{equation}
  \mathfrak{L}^\textrm{C}_n \,=\, f\bigl(\mathbf{X}_n[t],\mathbf{W}^\textrm{C}_n[t-1],\mathbf{W}^\textrm{S}[t-1]\bigr).
  \label{eq:sys-loss-c}
\end{equation}
The global loss combines both views and is given by the sample-weighted average:
\begin{equation}
  \mathfrak{L} \,=\, \frac{1}{2}\sum_{n=1}^{N}\frac{|D_n|}{D}\,(\mathfrak{L}^\textrm{C}_n + \mathfrak{L}^\textrm{S}).
\end{equation}

% Let $\mathbf{W}^S[t]$ denote the trainable server-side parameters, $\mathbf{W}[t]$ be the all trainable parameters at round $t$. Also, let $|D_n|$ be the sample size of terminal $n$ and let $D$ be the total number of samples. The global loss is
% \begin{equation}
%   L(\mathbf{W}) \,=\, \sum_{n=1}^{N}\frac{|D_n|}{D}\,L^C_n(\mathbf{W}),
%   \label{eq:sys-obj}
% \end{equation}
% The server-side update is
% \begin{equation}
%   \mathbf{W}^S[t] \,=\, \mathbf{W}^S[t-1]-\eta^S\,\mathbf{G}^S[t],
%   \label{eq:sys-upd-s}
% \end{equation}
% and the terminal-side update is
% \begin{equation}
%   \mathbf{W}^C_n[t] \,=\, \mathbf{W}^C_n[t-1]-\eta^C\,\mathbf{G}^C_n[t],
%   \label{eq:sys-upd-c}
% \end{equation}
% where $\eta^S$ and $\eta^C$ are the learning rates, and $\mathbf{G}^S[t]$ and $\mathbf{G}^C_n[t]$ are the corresponding gradients. 
% At round $t$, terminal $n$ uses layer $l_n[t]$ as its last local layer. The terminal trains the model from the input to layer $l_n[t]$, and the server computes the remaining layers. Each scheduled terminal processes its local batch samples through its local layers and generates the split-layer activation:
% \begin{equation}
%   \mathbf{S}_n[t] \,=\, f\bigl(\mathbf{X}_n[t];\,\mathbf{W}^C_n[t-1]\bigr),
%   \label{eq:sys-Sfwd}
% \end{equation}
% where $\mathbf{W}^C_n[t-1]$ denotes the trainable parameters on the client (terminal) side. The activation is compressed with level $\rho_n[t]$ and uploaded to the BS together with the labels. The server then continues the model training on the remaining layers, computes the loss, and obtains the corresponding gradients. The server also updates the server-side trainable parameters. Next, it compresses the gradient at the split layer with the same level and sends the result back to the terminal for local back-propagation.

% Let $W_s[t]$ denote the trainable server-side parameters. Let $W[t]$ collect all trainable parameters at round $t$. Also, let $|\mathcal{D}_n|$ be the sample size of terminal $n$ and let $D$ be the total number of samples. The global loss is
% \begin{equation}
%   L(W) \,=\, \sum_{n=1}^{N}\frac{|\mathcal{D}_n|}{D}\,L_n(W),
%   \label{eq:sys-obj}
% \end{equation}
% The server-side update is
% \begin{equation}
%   W_s[t] \,=\, W_s[t-1]-\eta_s\,\mathbf{G}_s[t],
%   \label{eq:sys-upd-s}
% \end{equation}
% and the terminal-side update is
% \begin{equation}
%   W_{c,n}[t] \,=\, W_{c,n}[t-1]-\eta_c\,\mathbf{G}_{c,n}[t],
%   \label{eq:sys-upd-c}
% \end{equation}
% where $\eta_s$ and $\eta_c$ are the learning rates, and $\mathbf{G}_s[t]$ and $\mathbf{G}_{c,n}[t]$ are the corresponding gradients. Let $F$ denote the aggregation interval.

% After every $F$ rounds, the terminal-side parameters are aggregated by sample-weighted federated averaging:
% Periodically, the server aggregates the terminal-side parameters of the scheduled terminals by sample-weighted federated averaging:
% \begin{equation}
%   \overline{\mathbf{W}}^C[t] \,=\, \sum_{n=1}^{N}\frac{|D_n|}{D}\mathbf{W}^C_n[t],
%   \label{eq:sys-fedavg}
% \end{equation}
% after which each $W_{c,n}[t]$ is replaced by $\overline{W}_c[t]$. For a candidate action $(j_n[t],\rho_n[t],m_n[t])_{n=1}^{N}$, the training sub-twin uses a model instance synchronized with the current model to simulate one round of training. It then outputs the resulting $\Delta\hat{L}[t]$. In this way, the BS can evaluate the short-term training effect of an action without sending data over the physical link.
The server periodically averages the client-side parameters. To do this, it weights each $\mathbf{W}^\textrm{C}_n[t]$ by the size of its local data set $|D_n|$. For a candidate action $(l_n[t],\rho_n[t])_{n=1}^{N}$, the training sub-twin simulates one round of training and outputs the predicted loss reduction $\mathfrak{L}$.

\subsection{Task Sub-Twin}
\label{sec:sys-task}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{results/task_twin.pdf }
    \caption{Task sub-twin illustration.}
    \label{fig:placeholder}
\end{figure}

% A candidate action cannot be checked freely through real task evaluation, because task success is only observed after expensive task assessments. 
% Evaluating a trained model directly on real equipment is unsafe, since a wrong training decision can drive the updated model to unsafe behavior and cause sudden damage before its task performance is observed.
% The task sub-twin $\widehat{\Omega}^{r}[t]$ estimates the task-level performance of the fine-tuned model. Let $\mathcal{E}$ denote a held-out set of evaluation episodes drawn from the deployment distribution. For episode $\tau\in\mathcal{E}$, let $\xi(W,\tau)\in\{0,1\}$ indicate whether the model with parameter $W$ completes the task successfully. The task success rate at round $t$ is
% \begin{equation}
%   A[t] \,=\, \frac{1}{|\mathcal{E}|}\sum_{\tau\in\mathcal{E}}\xi\bigl(W[t],\tau\bigr),
%   \label{eq:sys-A}
% \end{equation}
% and the corresponding improvement is $\Delta A[t]\triangleq A[t]-A[t-1]$ for $t\in\mathcal{R}$.

% Computing $A[t]$ requires running evaluation episodes in the task environment. Doing this in every round is too expensive. The task sub-twin therefore evaluates $W[t]$ in a virtual version of the deployment environment~\cite{Liu2023NeurIPS} and returns a per-round estimate $\hat{A}[t]$. This estimate provides frequent task-level feedback without requiring full physical evaluation in every round.
Evaluating a trained model directly on real equipment is unsafe, since a wrong training decision can drive the updated model to unsafe behavior and cause sudden damage before its task performance is observed.
The task sub-twin $\widehat{\Omega}^{T}[t]$ estimates the task-level performance of the fine-tuned model. Let $\mathcal{E}$ denote a held-out set of evaluation episodes drawn from the deployment distribution. For episode $\tau\in\mathcal{E}$, let $\xi(\mathbf{W},\tau)\in\{0,1\}$ indicate whether the model with parameter $\mathbf{W}$ completes the task successfully. The task success rate at round $t$ is
\begin{equation}
  A[t] \,=\, \frac{1}{|\mathcal{E}|}\sum_{\tau\in\mathcal{E}}\xi\bigl(\mathbf{W}[t],\tau\bigr),
  \label{eq:sys-A}
\end{equation}
and the corresponding improvement is $\Delta A[t]\triangleq A[t]-A[t-1]$ for $t\in\{1,\dots,T\}$.
Computing $A[t]$ requires running evaluation episodes in the task environment. Doing this in every round is too expensive. The task sub-twin therefore evaluates $\mathbf{W}[t]$ in a virtual version of the deployment environment~\cite{Liu2023NeurIPS} and returns a per-round estimate $\hat{A}[t]$, and thus providing frequent task-level feedback without requiring full physical evaluation in every round.

\subsection{Problem Formulation}
\label{sec:prob}

% Before formulating the optimization problem, we first compose the outputs of the three sub-twins into per-round expressions for latency, energy consumption, and memory usage. Let $\psi(j)$ denote the per-sample size of the split-layer activation when the model is split at layer $j$. Let $\varphi(j)$ and $\varpi(j)$ denote the per-sample forward and backward computational workloads of the on-device front sub-model. Under the action $(b_n[t],p_n[t],j_n[t],\rho_n[t])$, the transmission delay on the split interface is
% \begin{equation}
%   \ell^{x}_n[t] \,=\, \frac{b\,\psi(j_n[t])\,(1-\rho_n[t])}{R^{x}_n[t]},\quad x\in\{u,d\},
%   \label{eq:sys-T}
% \end{equation}
% for both uplink and downlink. The on-device computation delay is
% \begin{equation}
%   \ell^{p}_n[t] \,=\, \frac{b\,\bigl[\varphi(j_n[t])+\varpi(j_n[t])\bigr]}{\nu_n\,f_n},
%   \label{eq:sys-Tp}
% \end{equation}
% where $\nu_n$ and $f_n$ are the operations per cycle and the processor frequency of terminal $n$, respectively.

% The round completion time is determined by the slowest scheduled terminal:
% \begin{equation}
%   \ell^{c}[t] \,=\, \max_{n\in\mathcal{S}[t]}\!\bigl(\ell^{p}_n[t]+\ell^{u}_n[t]+\ell^{d}_n[t]\bigr),
%   \label{eq:sys-TC}
% \end{equation}
% that is, a round finishes only after the slowest scheduled terminal completes its local computation, uplink transmission, and downlink reception.

% The total energy consumption of terminal $n$ in round $t$ is
% \begin{equation}
%   E_n[t] \,=\, \kappa_n\,f_n^{\,2}\,b\,\bigl[\varphi(j_n[t])+\varpi(j_n[t])\bigr] + p_n[t]\,\ell^{u}_n[t],
%   \label{eq:sys-E}
% \end{equation}
% where $\kappa_n$ is a hardware-dependent coefficient. Finally, let $M_n(j)$ denote the total on-device memory required when the model is split at layer $j$. This includes the front sub-model, its optimizer state, and the cached activations. This quantity must satisfy the terminal memory budget $\bar{M}_n$.
Before formulating the optimization problem, we first compose the outputs of the three sub-twins into per-round expressions for latency, energy consumption, and memory usage. Let $\psi(l)$ denote the per-sample size of the split-layer activation when the model is split at layer $l$, and let $\varphi(l)$ denote the per-sample computational workload of the on-device front sub-model. Let $\mathcal{S}[t]\triangleq\{n:\alpha_n[t]=1\}$ be the terminals scheduled in round $t$. Under the action $(\mathrm{b}_n[t],\mathrm{p}_n[t],l_n[t],\rho_n[t])$, since the gradient at the split layer has the same dimension as the corresponding activation, the uplink and downlink share a common per-direction transmission delay
\begin{equation}
  \delta^{\textrm{Tx}}_n[t] \,=\, \frac{|D_n|\,\psi(l_n[t])\,(1-\rho_n[t])}{R_n[t]}.
  \label{eq:sys-T}
\end{equation}
The on-device computation delay is
\begin{equation}
  \delta^{\textrm{Cp}}_n[t] \,=\, \frac{|D_n|\,\varphi(l_n[t])}{\nu_n\,g_n},
  \label{eq:sys-Tp}
\end{equation}
where $\nu_n$ and $g_n$ are the operations per cycle and the processor frequency of terminal $n$, respectively.
The round completion time is determined by the slowest scheduled terminal:
\begin{equation}
  \delta[t] \,=\, \max_{n\in\mathcal{S}[t]}\!\bigl(\delta^{\textrm{Cp}}_n[t]+2\,\delta^{\textrm{Tx}}_n[t]\bigr),
  \label{eq:sys-TC}
\end{equation}
that is, a round finishes only after the slowest scheduled terminal completes its local computation, uplink transmission, and downlink reception.
The total energy consumption of terminal $n$ in round $t$ is
\begin{equation}
  E_n[t] \,=\, \kappa_n\,g_n^{\,2}\,|D_n|\,\varphi(l_n[t]) + \mathrm{p}_n[t]\,\delta^{\textrm{Tx}}_n[t],
  \label{eq:sys-E}
\end{equation}
where $\kappa_n$ is a hardware-dependent coefficient~\cite{Yang2021TWC}. 

Let $\textrm{m}_n(l)$ denote the total on-device memory required when the model is split at layer $l$. This includes the front sub-model, its optimizer state, and the cached activations. This quantity must satisfy the terminal memory budget $\bar{\mathrm{M}}_n$.

% \begin{table}[!t]
%   \centering
%   \caption{Summary of Important Notations.}
%   \label{tab:notation}
%   \renewcommand{\arraystretch}{1.15}
%   \setlength{\tabcolsep}{4pt}
%   \small
%   \begin{tabular}{@{}p{0.22\linewidth}p{0.74\linewidth}@{}}
%     \toprule
%     \textbf{Symbol} & \textbf{Description}\\
%     \midrule
%     $N,\,\mathcal{N}$ & Number and index set of terminals \\
%     $\Phi$ & Shared foundation model \\
%     $R,\,\mathcal{R}$ & Total training rounds and the corresponding set \\
%     $\gamma$ & Discount factor \\
%     $\bar{\ell}$ & Per-round deadline \\
%     $f_c,\,N_0$ & Carrier frequency and noise power spectral density \\
%     $a[t],\,\mathcal{A}[t]$ & Per-round joint action and feasible action set \\
%     $\mathcal{S}[t]$ & Set of scheduled terminals in round $t$ \\
%     $b_n[t],\,B$ & Per-terminal bandwidth allocation and total budget \\
%     $p_n[t],\,\bar{P}$ & Transmit power and its per-terminal budget \\
%     $j_n[t],\,\mathcal{K}$ & Last local layer and admissible layer set \\
%     $\rho_n[t],\,\bar{\rho}$ & Compression level and its upper bound \\
%     $m_n[t]$ & Scheduling indicator of terminal $n$ \\
%     $b$ & Per-terminal mini-batch size \\
%     $G_n$ & Large-scale channel gain of terminal $n$ \\
%     $H_n[t]$ & Small-scale fading coefficient of terminal $n$ \\
%     $\mathbf{x}_n,\,\mathfrak{e}$ & Terminal location and propagation environment \\
%     $f_D,\,\rho_H$ & Doppler shift and temporal fading correlation \\
%     $R^{u}_n[t],\,R^{d}_n[t]$ & Uplink and downlink maximum transmission rates \\
%     $\mathbf{X}_n[t],\,\mathbf{S}_n[t]$ & Local input batch and split-layer activation \\
%     $W[t]$ & Trainable parameters at round $t$ \\
%     $W_{c,n}[t],\,W_s[t]$ & Terminal- and server-side trainable parameters \\
%     $\overline{W}_c[t]$ & Federated-averaged terminal-side parameters \\
%     $F$ & Federated aggregation interval \\
%     $\eta_c,\,\eta_s$ & Terminal- and server-side learning rates \\
%     $\mathbf{G}_{c,n}[t],\,\mathbf{G}_s[t]$ & Terminal- and server-side gradients \\
%     $L(W),\,L_n(W)$ & Global and per-terminal training loss \\
%     $\mathcal{D}_n,\,D$ & Local dataset of terminal $n$ and total sample count \\
%     $\Delta\hat{L}[t]$ & Twin-predicted one-round loss reduction \\
%     $\mathcal{E},\,\xi(W,\tau)$ & Evaluation episode set and per-episode success indicator \\
%     $A[t],\,\Delta A[t]$ & Task success rate and its per-round improvement \\
%     $\hat{A}[t]$ & Twin-estimated task success rate \\
%     $\psi(j)$ & Per-sample size of the split-layer activation \\
%     $\varphi(j),\,\varpi(j)$ & Per-sample forward and backward compute workloads \\
%     $\ell^{u}_n[t],\,\ell^{d}_n[t]$ & Uplink and downlink transmission delay \\
%     $\ell^{p}_n[t],\,\ell^{c}[t]$ & On-device compute delay and round completion time \\
%     $\nu_n,\,f_n$ & Operations per cycle and processor frequency of terminal $n$ \\
%     $\kappa_n$ & Hardware-dependent energy coefficient \\
%     $E_n[t]$ & Total energy consumption of terminal $n$ in round $t$ \\
%     $M_n(j),\,\bar{M}_n$ & On-device memory usage and memory budget \\
%     $\widehat{\Omega}[t]$ & Cross-domain digital twin \\
%     $\widehat{\Omega}^{w},\,\widehat{\Omega}^{l},\,\widehat{\Omega}^{r}$ & Network, training, and task sub-twins \\
%     \bottomrule
%   \end{tabular}
% \end{table}

At round $t\in\{1,\dots,T\}$, the BS jointly chooses the action $a[t]\in\mathcal{A}[t]$, where $\mathcal{A}[t]$ is the feasible action set defined by the physical constraints below. Let $\bar{\delta}$ denote the per-round deadline, $\bar{\mathrm{B}}$ the total bandwidth budget, and $\mathcal{L}\triangleq\{1,\dots,L\}$ the set of admissible split-layer indices, where $L$ is the total number of layers of $\Phi$. With discount factor $\gamma\in(0,1)$, we formulate the following optimization problem:
\begin{equation}
\begin{split}
  (\mathrm{P_1}):\;\;\max_{\{a[t]\}}\;& \mathbb{E}\!\Bigl[\sum_{t=1}^{T}\gamma^{\,t-1}\bigl(A[t]-A[t-1]\bigr)\Bigr] \\
  \mathrm{s.t.}\;\;
  & (\mathrm{C}_1):\; \delta^{\textrm{Cp}}_n[t]+2\,\delta^{\textrm{Tx}}_n[t]\le\bar{\delta},\\
  & (\mathrm{C}_2):\; \textrm{m}_n(l_n[t])\le\bar{\mathrm{M}}_n,\\
  & (\mathrm{C}_3):\; \textstyle\sum_{n}\mathrm{b}_n[t]\le\bar{\mathrm{B}},\\
  & (\mathrm{C}_4):\; 0\le\mathrm{p}_n[t]\le\bar{\mathrm{P}},\\
  & (\mathrm{C}_5):\; 0\le\rho_n[t]\le\bar{\rho},\\
  & (\mathrm{C}_6):\; l_n[t]\in\mathcal{L},\;\;\alpha_n[t]\in\{0,1\},\\
  & (\mathrm{C}_7):\; \textstyle\sum_{n}\alpha_n[t]\ge 1.
  \label{eq:prob-P}
\end{split}
\end{equation}
Constraint $(\mathrm{C}_1)$ enforces the per-round deadline. Constraint $(\mathrm{C}_2)$ enforces the memory limit of each terminal. Constraint $(\mathrm{C}_3)$ enforces the total bandwidth budget. Constraint $(\mathrm{C}_7)$ excludes the degenerate case in which no terminal is scheduled, i.e., $\alpha_n[t]=0$ for all $n$, under which the maximum in~\eqref{eq:sys-TC} would be undefined. The remaining constraints bound the continuous and discrete decision variables.

Problem $(\mathrm{P_1})$ presents two main challenges. First, the objective increment $\Delta A[t]$ cannot be expressed in closed form as a function of $\mathbf{a}[t]$. Its value depends on the training trajectory $\{\mathbf{W}[t']\}_{t'\le t}$ produced by the FSL dynamics in~\eqref{eq:sys-Sfwd}--\eqref{eq:sys-upd-c}, so it must be estimated through task evaluation. Second, $\mathbf{a}[t]$ includes variables that operate on distinct time scales. The variables $(\mathrm{b}_n[t],\mathrm{p}_n[t])$ respond to rapid wireless fluctuations, while $(l_n[t],\rho_n[t],\alpha_n[t])$ influence the slower progression of model training and task performance. These challenges motivate a round-by-round solution for $(\mathrm{P_1})$, using $\widehat{\Omega}[t]$ as an evaluation proxy. The details of this approach are developed in the next section.

% Problem $(\mathrm{P_1})$ is difficult for two reasons. First, the objective increment $\Delta A[t]$ is not available in closed form as a function of $\mathbf{a}[t]$. It depends on the training trajectory $\{\mathbf{W}[t']\}_{t'\le t}$ generated by the FSL dynamics in~\eqref{eq:sys-Sfwd}--\eqref{eq:sys-upd-c}, and must therefore be estimated through task evaluation. Second, $\mathbf{a}[t]$ contains variables that operate on different time scales: $(\mathrm{b}_n[t],\mathrm{p}_n[t])$ respond to fast wireless fluctuations, while $(l_n[t],\rho_n[t],\alpha_n[t])$ shape the slower evolution of model training and task success. These two properties motivate solving $(\mathrm{P_1})$ in a round-by-round manner with $\widehat{\Omega}[t]$ as the evaluation substitute, which we develop in the next section.
% Let $\mathcal{R}\triangleq\{1,\ldots,R\}$ denote the set of training rounds. At round $t\in\mathcal{R}$, the controller jointly chooses the five control variables of all terminals. This yields the $5N$-dimensional mixed-integer action $a[t]\triangleq\bigl(b_n[t],p_n[t],j_n[t],\rho_n[t],m_n[t]\bigr)_{n=1}^{N}\in\mathcal{A}[t]$. Here, $\mathcal{A}[t]$ is the feasible action set defined by the physical constraints below. With discount factor $\gamma\in(0,1)$, we formulate the following optimization problem:
% \begin{equation}
% \begin{split}
%   (\mathrm{P_1}):\;\;\max_{\{a[t]\}}\;& \mathbb{E}\!\Bigl[\sum_{t=1}^{R}\gamma^{\,t-1}\bigl(A[t]-A[t-1]\bigr)\Bigr] \\
%   \mathrm{s.t.}\;\;
%   & (\mathrm{C}_1):\; \ell^{p}_n[t]+\ell^{u}_n[t]+\ell^{d}_n[t]\le\bar{\ell},\\
%   & (\mathrm{C}_2):\; M_n(j_n[t])\le\bar{M}_n,\\
%   & (\mathrm{C}_3):\; \textstyle\sum_{n}b_n[t]\le B,\\
%   & (\mathrm{C}_4):\; 0\le p_n[t]\le\bar{P},\\
%   & (\mathrm{C}_5):\; 0\le\rho_n[t]\le\bar{\rho},\\
%   & (\mathrm{C}_6):\; j_n[t]\in\mathcal{K},\;\;m_n[t]\in\{0,1\},\\
%   & (\mathrm{C}_7):\; \textstyle\sum_{n}m_n[t]\ge 1.
%   \label{eq:prob-P}
% \end{split}
% \end{equation}
% Constraint $(\mathrm{C}_1)$ enforces the per-round deadline. Constraint $(\mathrm{C}_2)$ enforces the memory limit of each terminal. Constraint $(\mathrm{C}_3)$ enforces the total bandwidth budget. Constraint $(\mathrm{C}_7)$ excludes the degenerate case in which no terminal is scheduled; otherwise, the maximum in~\eqref{eq:sys-TC} and the denominator in~\eqref{eq:sys-fedavg} would be undefined. The remaining constraints bound the continuous and discrete decision variables.

% Problem $(\mathrm{P_1})$ is difficult for two reasons. First, the objective increment $\Delta A[t]$ is not available in closed form as a function of $a[t]$. It depends on the training trajectory $\{W[t']\}_{t'\le t}$ generated by the FSL dynamics in~\eqref{eq:sys-Sfwd}--\eqref{eq:sys-fedavg}. It must therefore be estimated through task evaluation. Second, the action contains variables that operate on different time scales. The variables $(b_n[t],p_n[t])$ respond to fast wireless fluctuations. The variables $(j_n[t],\rho_n[t],m_n[t])$ shape the slower evolution of model training and task success. These two properties motivate the twin-assisted sequential decision framework, where $\widehat{\Omega}[t]$ is used as the evaluation substitute of $(\mathrm{P_1})$ for round-by-round planning.


==> section/4.TheoreticalAnalysis.tex <==
%% =====================================================================
%%  Section 4 : Theoretical Analysis
%% =====================================================================
\section{Theoretical Analysis}
\label{sec:analysis}

Under the stipulation that the FSL training loop of Eqs.~\eqref{eq:sys-upd-s} and~\eqref{eq:sys-upd-c} is parametrized by $(q^{\max},\{x_n[t]\},F)$, we bound the non-convex surrogate $\min_{t\le T}\mathbb{E}\|\nabla\mathcal{J}(\mathbf{W}[t])\|^{2}$ explicitly in these three coordinates.

The analysis rests on the conventional triple of assumptions: (i) each $\mathcal{J}_n(\mathbf{W})$ is $\beta$-smooth and the gradients $\mathbf{G}^{\mathrm{c}}_n[t],\mathbf{G}^{\mathrm{s}}_n[t]$ are unbiased with variance bounded by $\sigma_g^{2}$; (ii) the cross-terminal dissimilarity satisfies $\frac{1}{N}\sum_{n}\|\nabla\mathcal{J}_n(\mathbf{W})-\nabla\mathcal{J}(\mathbf{W})\|^{2}\le\zeta^{2}$; (iii) $\widetilde{\mathbf{G}}[t]$ induced by $\mathcal{S}[t]$ and the compression operator at $q_n[t]\le q^{\max}$ exhibits scheduling drift bounded by $\sigma_s^{2}$.

\begin{theorem}[FSL Convergence under Action Variables]
\label{thm:fsl-conv}
Under the stipulated assumptions, with $\eta=\Theta(1/\sqrt{NT})$ and federated aggregation every $F$ rounds over $T$ rounds, the FSL iterates satisfy
\begin{equation}
  \min_{t\le T}\,\mathbb{E}\bigl\|\nabla\mathcal{J}(\mathbf{W}[t])\bigr\|^{2}
  \;\le\;
  \frac{\Lambda_0}{\sqrt{NT}}
  +\Lambda_1(q^{\max})^{2}
  +\Lambda_2 F\sigma_s^{2},
  \label{eq:ana-fsl-conv}
\end{equation}
where $\Lambda_0,\Lambda_1,\Lambda_2$ depend on $\beta,\sigma_g^{2},\zeta^{2}$.
\end{theorem}

\begin{proof}[Proof sketch]
Writing $\mathcal{J}_t\triangleq\mathcal{J}(\mathbf{W}[t])$, the $\beta$-smooth descent lemma applied to $\mathbf{W}[t+1]-\mathbf{W}[t]=-\eta\widetilde{\mathbf{G}}_t$ under $\eta\le 1/\beta$ yields $\mathbb{E}[\mathcal{J}_{t+1}-\mathcal{J}_t]\le -\tfrac{\eta}{2}\mathbb{E}\|\nabla\mathcal{J}_t\|^{2}+\tfrac{\eta^{2}\beta}{2}\mathbb{E}\|\widetilde{\mathbf{G}}_t\|^{2}$. Decomposing $\widetilde{\mathbf{G}}_t$ into stochastic-gradient noise ($\sigma_g^{2}/N$), heterogeneity ($\zeta^{2}$), quantization ($\propto (q^{\max})^{2}$), and $F$-round scheduling drift ($\sigma_s^{2}$) bounds its second moment by $\|\nabla\mathcal{J}_t\|^{2}+\Sigma_F$ with $\Sigma_F\triangleq\sigma_g^{2}/N+\zeta^{2}+c_q(q^{\max})^{2}+F\sigma_s^{2}$. Telescoping over $T$ rounds and balancing $\eta=\Theta(1/\sqrt{NT})$ substantiates Eq.~\eqref{eq:ana-fsl-conv}.
\end{proof}

\begin{theorem}[Twin-Induced Reward Error]
\label{thm:twin-reward}
The per-round reward $r[t]$ of Eq.~\eqref{eq:method-reward} is an affine functional of the twin-observable quantities $\bigl(\widehat{\delta}[t],\{\widehat{E}_n[t],\widehat{\delta}^{\mathrm{cp}}_n[t],\widehat{\delta}^{\mathrm{tx}}_n[t]\}_{n\in\mathcal{S}[t]},\Delta\widehat{\Gamma}[t]\bigr)$, with coefficients determined by $w_{\delta},w_E,w_{\mathrm{pen}}$ of Eqs.~\eqref{eq:method-r-comm} to~\eqref{eq:method-violation}. Let $\epsilon_{\mathrm{cal}}[t]$ denote the $\ell_1$-aggregated calibration discrepancy between these twin-observable quantities and their physical counterparts at round $t$. Then the twin-estimated reward $\widehat r[t]$ satisfies
\begin{equation}
  \mathbb{E}\bigl|\widehat r[t]-r[t]\bigr|
  \;\le\;
  \Lambda_r\,\epsilon_{\mathrm{cal}}[t],
  \label{eq:ana-reward-error}
\end{equation}
with $\Lambda_r\triangleq\max\{w_{\delta}/\delta^{\max},w_E/E^{\max},1,w_{\mathrm{pen}}\}$.
\end{theorem}

\begin{proof}[Proof sketch]
Substituting Eqs.~\eqref{eq:method-r-task} to~\eqref{eq:method-violation} into Eq.~\eqref{eq:method-reward} renders $r[t]$ affine in $\bigl(\widehat{\delta},\{\widehat{E}_n\},\Delta\widehat{\Gamma}\bigr)$ with coefficients $w_{\delta}/\delta^{\max}, w_E/E^{\max}, 1$, plus a $w_{\mathrm{pen}}$-weighted penalty piecewise-linear in $\{\widehat{\delta}^{\mathrm{cp}}_n,\widehat{\delta}^{\mathrm{tx}}_n\}$. Triangle inequality along each coordinate, aggregated under $\Lambda_r$ and expectation under $\epsilon_{\mathrm{cal}}[t]$, substantiates Eq.~\eqref{eq:ana-reward-error}.
\end{proof}

% \begin{remark}
Theorem~\ref{thm:fsl-conv} bounds how $q_n[t]$ and $x_n[t]$ shape the training-loss floor through $\Lambda_1(q^{\max})^{2}$ and $\Lambda_2 F\sigma_s^{2}$. Theorem~\ref{thm:twin-reward} bounds how the three calibration loops shape the planning quality: as $\epsilon_{\mathrm{cal}}[t]\to 0$, the CEM ranking inside the twin aligns with that under the true environment, substantiating $\widehat r[t]$ as TiLP's planning surrogate.
% \end{remark}


==> section/4_analysis.tex <==
%% =====================================================================
%%  Section 4 : Theoretical Analysis
%% =====================================================================
\section{Theoretical Analysis}
\label{sec:analysis}

This section is predicated on the stipulation that the FSL training loop of Eqs.~\eqref{eq:sys-upd-s} and~\eqref{eq:sys-upd-c} is parametrized by the configuration $(\bar q,\{x_n[t]\},F)$, with the achievable optimization quality scrutinized against perturbations of these three coordinates. Because $\mathcal{J}(\mathbf{W})$ is non-convex under the foundation-model parametrization, we adopt the standard surrogate $\min_{t\le R}\mathbb{E}\|\nabla\mathcal{J}(\mathbf{W}[t])\|^{2}$ as the progress measure and bound it explicitly in $(\bar q,\{x_n[t]\},F)$.

The analysis rests on the conventional triple of assumptions: (i) each $\mathcal{J}_n(\mathbf{W})$ is $\beta$-smooth and the gradients $\mathbf{G}^{\mathrm{c}}_n[t],\mathbf{G}^{\mathrm{s}}[t]$ are unbiased with variance bounded by $\sigma_g^{2}$; (ii) the cross-terminal dissimilarity satisfies $\frac{1}{N}\sum_{n}\|\nabla\mathcal{J}_n(\mathbf{W})-\nabla\mathcal{J}(\mathbf{W})\|^{2}\le\zeta^{2}$; (iii) $\widetilde{\mathbf{G}}[t]$ induced by $\mathcal{S}[t]$ and the compression operator at $q_n[t]\le\bar q$ exhibits scheduling drift bounded by $\sigma_s^{2}$.

\begin{theorem}[FSL Convergence under Action Variables]
\label{thm:fsl-conv}
Under the stipulated assumptions, with $\eta=\Theta(1/\sqrt{NR})$ and federated aggregation every $F$ rounds over $R$ rounds, the FSL iterates satisfy
\begin{equation}
  \min_{t\le R}\,\mathbb{E}\bigl\|\nabla\mathcal{J}(\mathbf{W}[t])\bigr\|^{2}
  \;\le\;
  \frac{\Lambda_0}{\sqrt{NR}}
  +\Lambda_1\bar q^{2}
  +\Lambda_2 F\sigma_s^{2},
  \label{eq:ana-fsl-conv}
\end{equation}
where $\Lambda_0,\Lambda_1,\Lambda_2$ depend on $\beta,\sigma_g^{2},\zeta^{2}$.
\end{theorem}

\begin{proof}[Proof sketch]
The $\beta$-smooth descent lemma applied to $\mathbf{W}[t+1]-\mathbf{W}[t]=-\eta\widetilde{\mathbf{G}}[t]$ decomposes $\widetilde{\mathbf{G}}[t]$ into four orthogonal components: stochastic-gradient noise, heterogeneity noise, quantization noise (variance $\le\bar q^{2}$ under standard dithering), and $F$-round scheduling drift (variance $\le\sigma_s^{2}$). Telescoping over $R$ rounds and balancing $\eta=\Theta(1/\sqrt{NR})$ substantiates Eq.~\eqref{eq:ana-fsl-conv}.
\end{proof}

Whereas Theorem~\ref{thm:fsl-conv} addresses the training-loss floor, the planning quality of TiLP further hinges on whether the twin-estimated reward $\widehat r[t]$ tracks the physical $r[t]$, which the next result quantifies in terms of the round-$t$ sub-twin calibration discrepancy.

\begin{theorem}[Twin-Induced Reward Error]
\label{thm:twin-reward}
The per-round reward $r[t]$ of Eq.~\eqref{eq:method-reward} is an affine functional of the twin-observable quantities $\bigl(\widehat{\delta}[t],\{\widehat{E}_n[t],\widehat{\delta}^{\mathrm{cp}}_n[t],\widehat{\delta}^{\mathrm{tx}}_n[t]\}_{n\in\mathcal{S}[t]},\Delta\widehat{\Gamma}[t]\bigr)$, with coefficients determined by $w_{\delta},w_E,w_{\mathrm{pen}}$ of Eqs.~\eqref{eq:method-r-comm} to~\eqref{eq:method-violation}. Let $\epsilon_{\mathrm{cal}}[t]$ denote the $\ell_1$-aggregated calibration discrepancy between these twin-observable quantities and their physical counterparts at round $t$. Then the twin-estimated reward $\widehat r[t]$ satisfies
\begin{equation}
  \mathbb{E}\bigl|\widehat r[t]-r[t]\bigr|
  \;\le\;
  \Lambda_r\,\epsilon_{\mathrm{cal}}[t],
  \quad
  \Lambda_r\triangleq\max\!\left\{\tfrac{w_{\delta}}{\delta^{\max}},\tfrac{w_E}{E^{\max}},1,w_{\mathrm{pen}}\right\}.
  \label{eq:ana-reward-error}
\end{equation}
\end{theorem}

\begin{proof}[Proof sketch]
Substituting Eqs.~\eqref{eq:method-r-task} to~\eqref{eq:method-violation} into Eq.~\eqref{eq:method-reward} renders $r[t]$ as an affine combination of the listed twin-observable arguments and a $w_{\mathrm{pen}}$-weighted nonnegative penalty. Triangle inequality along each coordinate, followed by aggregation under the coordinate-wise Lipschitz constant $\Lambda_r$, substantiates Eq.~\eqref{eq:ana-reward-error}.
\end{proof}

\begin{remark}
Theorem~\ref{thm:fsl-conv} bounds how $q_n[t]$ and $x_n[t]$ shape the training-loss floor through $\Lambda_1\bar q^{2}$ and $\Lambda_2 F\sigma_s^{2}$. Theorem~\ref{thm:twin-reward} bounds how the three calibration loops shape the planning quality: as $\epsilon_{\mathrm{cal}}[t]\to 0$, the CEM ranking inside the twin aligns with that under the true environment, substantiating $\widehat r[t]$ as TiLP's planning surrogate.
\end{remark}


==> section/5_method_design.tex <==
%% =====================================================================
%%  Section 5 : Method Design
%% =====================================================================
\section{TiLP: Twin-in-the-Loop Planner}
\label{sec:method}
We propose TiLP, which casts $(\mathrm{P_1})$ as an MDP and plans each round's $a[t]$ by cross-entropy method (CEM)~\cite{Rubinstein1999} receding-horizon search inside the twin $\widehat{\Omega}[t]$. The three sub-twins $\widehat{\Omega}_1,\widehat{\Omega}_2,\widehat{\Omega}_3$ are kept faithful by three multi-scale calibration loops, running at the per-round, per-aggregation, and per-evaluation.
% Problem~$(\mathrm{P_1})$ cannot be solved directly, because $\Delta A[t]$ has no closed form in $a[t]$ and is observable only through stochastic federated split learning (FSL) dynamics and a costly task rollout. We therefore cast it as a Markov decision process (MDP) and adopt model-based reinforcement learning (MBRL), using the cross-domain digital twin $\widehat{\Omega}[t]$ as a world model that scores candidate actions without invoking the physical system. The twin is composed of three sub-twins $(\widehat{\Omega}^w,\widehat{\Omega}^l,\widehat{\Omega}^r)$ instead of a single end-to-end learned dynamics model, because the three physical processes (channel fading, FSL training, and task rollout) operate on different time scales. Each sub-twin maintains its own intrinsic parameters $\boldsymbol{\Psi}\triangleq(\boldsymbol{\Psi}^w,\boldsymbol{\Psi}^l,\boldsymbol{\Psi}^r)$, refreshed at the corresponding cadence. Per-round decisions are produced by the cross-entropy method (CEM)~\cite{Rubinstein1999}, which natively scores the mixed continuous-discrete candidates in $a[t]$. A parametric actor--critic is trained alongside CEM to provide a warm-start prior and a terminal value; at deployment, the actor alone can be queried when CEM is too expensive.

\subsection{Cross-Domain Sub-Twins}
\label{sec:method-wm}

% The DT $\widehat{\Omega}[t]$ takes the current state $s[t]$ and a candidate action $a[t]$ and returns the per-round reward of Eq.~\eqref{eq:method-reward} together with the next observations. Three sub-twins split this prediction by action block: $\widehat{\Omega}^{N}$ handles the wireless variables, $\widehat{\Omega}^{L}$ the split-learning variables, and $\widehat{\Omega}^{T}$ the task readout.

% The DT $\widehat{\Omega}[t]$ takes the current state $s[t]$ and a candidate action $a[t]$ and predicts the per-round reward defined in Eq.~\eqref{eq:method-reward}. The prediction relies on three cross-domain sub-twin action blocks: $\widehat{\Omega}^{N}$ processes network variables, $\widehat{\Omega}^{L}$ handles learning variables, and $\widehat{\Omega}^{T}$ manages the task readout.

% The network sub-twin $\widehat{\Omega}^{N}$ takes the wireless variables $(\mathrm{b}_n[t],\mathrm{p}_n[t])$ and the network observation $o^{N}[t]$, and returns the predicted rate $\hat{R}_n[t]$, round latency $\hat{\delta}[t]$, and per-agent energy $\hat{E}_n[t]$ via Eqs.~\eqref{eq:sys-R}, \eqref{eq:sys-TC}, and \eqref{eq:sys-E}. Its parameters $\boldsymbol{\Psi}^{N}[t]$ carry the small-scale fading statistics and per-device energy coefficients left unspecified by the closed forms. Loop 1 fires once per round and fits $\boldsymbol{\Psi}^{N}[t]$ to the residual between the predicted $(\hat{\delta},\hat{E}_n)$ and the realized $(\delta,E_n)$.

% The training sub-twin $\widehat{\Omega}^{L}$ takes the split-learning variables $(l_n[t],\rho_n[t],\alpha_n[t])$ and the learning observation $o^{L}[t]$, and returns the predicted one-round loss decrease $\Delta\hat{\mathfrak{L}}[t]$ through a lightweight parametric regressor with parameters $\boldsymbol{\Psi}^{L}[t]$. Loop 2 fires at every federated-averaging instant and refits $\boldsymbol{\Psi}^{L}[t]$ on a sliding window of the realized $\{\Delta\mathfrak{L}[\tau]\}$ together with their corresponding split-learning inputs.

% The task sub-twin $\widehat{\Omega}^{T}$ returns the success-rate estimate $\hat{A}[t]$ in two modes. During planning it reads off the cached value parameterized by $\boldsymbol{\Psi}^{T}[t]$. During evaluation the current $\mathbf{W}[t]$ is rolled out on the LIBERO manipulation benchmark~\cite{Liu2023NeurIPS} to obtain the true $A[t]$ via Eq.~\eqref{eq:sys-A}, and Loop 3 refreshes $\boldsymbol{\Psi}^{T}[t]$ on the residual between $\hat{A}[t]$ and $A[t]$.

The DT $\widehat{\Omega}[t]$ takes the current state $s[t]$ and a candidate action $a[t]$ and predicts the per-round reward defined in Eq.~\eqref{eq:method-reward}. Throughout this subsection, hatted quantities denote predicted values. The prediction relies on three cross-domain sub-twin action blocks: $\widehat{\Omega}_1$ processes network variables, $\widehat{\Omega}_2$ handles learning variables, and $\widehat{\Omega}_3$ manages the task readout.

The network sub-twin $\widehat{\Omega}_1$ takes the wireless variables $(\mathrm{b}_n[t],\mathrm{p}_n[t])$ and the network observation $o^{\textrm{N}}[t]$, and returns the predicted rate $\hat{R}_n[t]$, round latency $\hat{\delta}[t]$, and per-agent energy $\hat{E}_n[t]$ via Eqs.~\eqref{eq:sys-R}, \eqref{eq:sys-TC}, and \eqref{eq:sys-E}. Its parameters $\boldsymbol{\Psi}_1[t]$ carry the small-scale fading statistics and per-device energy coefficients left unspecified by the closed forms. Loop 1 fires once per round and fits $\boldsymbol{\Psi}_1[t]$ to the residual between the predicted $(\hat{\delta},\hat{E}_n)$ and the realized $(\delta,E_n)$.

The training sub-twin $\widehat{\Omega}_2$ takes the split-learning variables $(l_n[t],\rho_n[t],\alpha_n[t])$ and the learning observation $o^{\textrm{L}}[t]$, and returns the predicted one-round loss decrease $\Delta\hat{\mathfrak{L}}[t]$ through a lightweight parametric regressor with parameters $\boldsymbol{\Psi}_2[t]$. Loop 2 fires at every federated-averaging instant and refits $\boldsymbol{\Psi}_2[t]$ on a sliding window of the realized $\{\Delta\mathfrak{L}[\tau]\}$ together with their corresponding split-learning inputs.

The task sub-twin $\widehat{\Omega}_3$ returns the success-rate estimate $\hat{A}[t]$ in two modes. During planning it reads off the cached value parameterized by $\boldsymbol{\Psi}_3[t]$. During evaluation the current $\mathbf{W}[t]$ is rolled out on the LIBERO manipulation benchmark~\cite{Liu2023NeurIPS} to obtain the true $A[t]$ via Eq.~\eqref{eq:sys-A}, and Loop 3 refreshes $\boldsymbol{\Psi}_3[t]$ on the residual between $\hat{A}[t]$ and $A[t]$.

\subsection{MDP Formulation}
\label{sec:method-mdp}

We model the entire twin $\widehat{\Omega}[t]$ as a finite-horizon MDP with horizon $T$, discount $\gamma$, and per-round action $a[t]$ all inherited verbatim from $(\mathrm{P_1})$. Of the twin's three layers, only the wireless and learning layers carry one-step state transitions, governed by Eq.~\eqref{eq:sys-R} and Eqs.~\eqref{eq:sys-upd-s}--\eqref{eq:sys-upd-c} respectively, whereas the task layer is a deterministic readout of the accumulated $\mathbf{W}[t]$ and enters the MDP only through the per-round reward $r[t]$ via $\Delta A[t]$. Augmenting this task gain with an equally-weighted communication-efficiency term (energy of Eq.~\eqref{eq:sys-E} and latency of Eq.~\eqref{eq:sys-TC}) and a soft penalty on $(\mathrm{C}_1)$--$(\mathrm{C}_3)$ yields $r[t]$, whose discounted return $\mathbb{E}\bigl[\sum_{t=1}^{T}\gamma^{t-1}r[t]\bigr]$ extends $(\mathrm{P_1})$'s task-only objective with balanced communication efficiency.
% Following the framing above, $(\mathrm{P_1})$ is represented as an MDP $(\mathcal{S},\mathcal{A},P,\gamma)$. The one-step transition kernel factorizes as
% \begin{equation}
%   P \triangleq P_l\circ P_w,
% \end{equation}
% where $P_w$ advances the wireless block under the channel model of Eqs.\eqref{eq:sys-Y}--\eqref{eq:sys-R}, and $P_l$ advances the learning block under the FSL update of Eqs.\eqref{eq:sys-upd-s}--\eqref{eq:sys-upd-c}. The task-success rate has no transition of its own and appears only in the reward signal through $\Delta A[t]$.

% The controller does not observe the full parameter vector $W[t]$. The MDP state is therefore defined using only the quantities directly accessible to the controller.

\subsubsection{State}

The state collects one observation block per sub-twin,
\begin{equation}
  s[t] \triangleq \bigl(o^{\textrm{N}}[t],\,o^{\textrm{L}}[t],\,o^{\textrm{T}}[t]\bigr).
  \label{eq:method-state}
\end{equation}
The network block $o^{\textrm{N}}[t]$ records the large-scale gains $\{G_n\}$, the instantaneous fading powers $\{|H_n[t]|^{2}\}$, and the previous-round bandwidth allocation $\{\mathrm{b}_n[t-1]\}$. The learning block $o^{\textrm{L}}[t]$ records the global loss $\mathfrak{L}(\mathbf{W}[t-1])$ and the per-agent client-side gradient norms $\{\|\mathbf{G}^{\textrm{C}}_n[t-1]\|\}$. The task block $o^{\textrm{T}}[t]$ records the latest success-rate estimate $\hat{A}[t-1]$.
% The MDP state $s[t]$ consists of three observable blocks and a time-progress scalar,
% \begin{equation}
%   s[t] = \bigl(o^w[t],\;o^l[t],\;o^r[t],\;t/R\bigr)\in\mathcal{S},
%   \label{eq:method-state}
% \end{equation}
% with each block matching one of the three layers of $(\mathrm{P_1})$. The wireless block $o^w[t]$ records the per-agent large-scale gain $G_n$, the instantaneous fading power $|H_n[t]|^{2}$, and the previous-round spectrum occupancy, so that rates and deadline feasibility can be evaluated. The learning block $o^l[t]$ records the global loss $L(W[t\!-\!1])$, the per-agent head-adapter gradient norms $\{\|\mathbf{G}_{c,n}[t\!-\!1]\|\}_{n=1}^{N}$, and the aggregation phase $(t\bmod F)$, from which the learning sub-twin predicts the one-step training gain. The task block $o^r[t]$ records the latest twin-estimated task-success rate $\hat{A}[t\!-\!1]$ as an indicator of current task-level progress; this entry is updated only when the L3 calibration loop runs (every $E_{\mathrm{eval}}$ rounds) and remains constant between updates. The scalar $t/R$ encodes the remaining training budget.

\subsubsection{Action}

The action $a[t]$ and its feasible set $\mathcal{A}[t]$ defined by $(\mathrm{C}_1)$--$(\mathrm{C}_7)$ are inherited verbatim from $(\mathrm{P_1})$. The salient feature for the BS is that $a[t]$ is a mixed continuous-discrete object: $(\mathrm{b}_n,\mathrm{p}_n,\rho_n)$ are continuous, $l_n\in\mathcal{L}$ is categorical, and $\alpha_n\in\{0,1\}$ is binary.
% The action $a[t]$ is identical to that in $(\mathrm{P_1})$, comprising the five per-agent decision variables $(j_n[t],b_n[t],p_n[t],\rho_n[t],m_n[t])_{n=1}^{N}$, with the feasible set $\mathcal{A}[t]$ defined by constraints $(\text{C}_1)$--$(\text{C}_6)$.

\subsubsection{Reward}

% The per-round reward gives equal weight to learning progress and communication efficiency, with constraint relaxation added as a soft penalty:
The per-round reward balances learning progress and communication efficiency with equal weight while softly penalizing constraint violations:
\begin{equation}
  r[t] = r_1[t]+r_2[t]+r_3[t].
  \label{eq:method-reward}
\end{equation}
The learning term $r_1[t]$ denotes the task-success increment $\Delta A[t]$ supplied online by $\widehat{\Omega}_3$, which reproduces the $(\mathrm{P_1})$ objective. The communication term measures the normalized headroom against the round deadline and against the worst-case round energy $\bar{E}\triangleq N\bar{\mathrm{P}}\bar{\delta}$,
% The learning term $r_1[t]$ denotes the task-success increment $\Delta A[t]$, which reproduces the $(\mathrm{P_1})$ objective and is supplied online by $\widehat{\Omega}^{T}$. The communication term measures the normalized headroom against the round deadline and the worst-case round energy $\bar{E}\triangleq N\bar{\mathrm{P}}\bar{\delta}$,
\begin{equation}
  r_2[t] = w_\delta\!\left(1 - \frac{\delta[t]}{\bar{\delta}}\right) + w_E\!\left(1 - \frac{\sum_{n=1}^{N}E_n[t]}{\bar{E}}\right),
  \label{eq:method-rp}
\end{equation}
so that staying well below the round latency of Eq.~\eqref{eq:sys-TC} and the per-round energy of Eq.~\eqref{eq:sys-E} contributes positively; the prices $w_E,w_\delta>0$ are calibrated so that $r_2[t]$ matches $r_1[t]$ in expectation under representative trajectories, granting learning progress and communication efficiency equal weight in the planner's objective. The term $r_3[t]$ denotes $-w_\Gamma\,\Gamma[t]$, which relaxes $(\mathrm{C}_1)$--$(\mathrm{C}_3)$ via the aggregate function
\begin{equation}
\begin{split}
  \Gamma[t] &= \sum_{n=1}^{N}\max\bigl(0,\,\delta^{\textrm{Cp}}_n[t]+2\delta^{\textrm{Tx}}_n[t]-\bar{\delta}\bigr)\\
  &\quad+\sum_{n=1}^{N}\max\bigl(0,\,\textrm{m}_n(l_n[t])-\bar{\mathrm{M}}_n\bigr)\\
  &\quad+\max\Bigl(0,\,\textstyle\sum_{n=1}^{N}\mathrm{b}_n[t]-\bar{\mathrm{B}}\Bigr),
\end{split}
\label{eq:method-gamma}
\end{equation}
covering the latency, memory, and bandwidth constraints respectively, and vanishing whenever no constraint is violated. The remaining constraints are enforced inside CEM. $(\mathrm{C}_4)$--$(\mathrm{C}_5)$ by clipping continuous samples to their feasible intervals, $(\mathrm{C}_6)$ by projecting $l_n[t]$ onto $\mathcal{L}$, and $(\mathrm{C}_7)$ by rejecting all-zero schedules. Under any feasible trajectory the three terms are non-negative, non-negative, and zero respectively, and the MDP objective $\max_{\pi}\mathbb{E}\bigl[\sum_{t=1}^{T}\gamma^{t-1}r[t]\bigr]$ extends $(\mathrm{P_1})$'s task-only objective with an equally-weighted communication-efficiency term, with the realized hard-constraint satisfaction reported by $\bar{\Gamma}$ of Eq.~\eqref{eq:metric-gamma-bar}.
% The per-round reward $r[t]$ aligns the MDP objective with $(\mathrm{P_1})$ and converts the hard inequality constraints into a tractable planning signal,
% \begin{equation}
%   r[t] = r^m[t]+r^p[t]+r^q[t].
%   \label{eq:method-reward}
% \end{equation}
% The task-gain term $r^m[t]$, defined as $\Delta A[t]$, corresponds directly to the $(\mathrm{P_1})$ objective and is estimated online by the task sub-twin. The communication-cost term
% \begin{equation}
%   r^p[t] = -\alpha\!\sum_{n=1}^{N}\!E_n[t]-\beta\,\ell^{c}[t]
%   \label{eq:method-rp}
% \end{equation}
% penalizes the energy consumption of Eq.\eqref{eq:sys-E} and the communication latency of Eq.\eqref{eq:sys-TC}. The constraint-penalty term $r^q[t]=-\lambda\,\Gamma[t]$ softens the inequality constraints $(\text{C}_1)$--$(\text{C}_3)$, where $\Gamma[t]$ aggregates the per-agent latency slack, the memory slack, and the spectrum-budget slack,
% \begin{align}
%   \Gamma[t] &= \sum_{n=1}^{N}\max\!\bigl(0,\,\ell^{p}_n[t]+\ell^{u}_n[t]+\ell^{d}_n[t]-\bar{\ell}\bigr)\nonumber\\
%   &\quad+\sum_{n=1}^{N}\max\!\bigl(0,\,M_n(j_n[t])-\bar{M}_n\bigr)\nonumber\\
%   &\quad+\max\!\Bigl(0,\,\sum_{n=1}^{N}b_n[t]-B\Bigr).
%   \label{eq:method-gamma}
% \end{align}
% The remaining constraints are enforced inside the planner: $(\text{C}_4)$--$(\text{C}_5)$ by clipping continuous CEM samples to their feasible intervals, $(\text{C}_6)$ by discrete projection, and $(\text{C}_7)$ by rejecting empty schedules. Together, $r^p[t]$ and $r^q[t]$ form a Lagrangian surrogate for the physical envelope of $(\mathrm{P_1})$, with $(\alpha,\beta,\lambda)$ as price coefficients on energy, latency, and constraint slack. Because $(\mathrm{P_1})$ is non-convex, this surrogate is not guaranteed to recover the global optimum, and the degree to which the executed trajectory satisfies the original constraints is reported by the realized slack $\bar{\Gamma}$ of Eq.~\eqref{eq:metric-gamma-bar}.
% The MDP objective is $\max_{\pi}\,\mathbb{E}\!\bigl[\sum_{t=1}^{R}\gamma^{t-1}r[t]\bigr]$, consistent with the discounted formulation of $(\mathrm{P_1})$.

% \subsection{Cross-Domain Sub-Twins}
% \label{sec:method-wm}

% The cross-domain twin $\widehat{\Omega}[t]$ takes the current state $s[t]$ and a candidate action $a[t]$ and returns the per-round reward of Eq.~\eqref{eq:method-reward} together with the next observation blocks. Its three sub-twins split this prediction by action block: $\widehat{\Omega}^{N}$ handles the wireless variables, $\widehat{\Omega}^{L}$ the split-learning variables, and $\widehat{\Omega}^{T}$ the task readout.

% The network sub-twin $\widehat{\Omega}^{N}$ takes the wireless variables $(\mathrm{b}_n[t],\mathrm{p}_n[t])$ and the network observation $o^{N}[t]$, and returns the predicted rate $\hat{R}_n[t]$, round latency $\hat{\delta}[t]$, and per-agent energy $\hat{E}_n[t]$ via Eqs.~\eqref{eq:sys-R}, \eqref{eq:sys-TC}, and \eqref{eq:sys-E}. Its parameters $\boldsymbol{\Psi}^{N}[t]$ carry the small-scale fading statistics and per-device energy coefficients left unspecified by the closed forms. Loop 1 fires once per round and fits $\boldsymbol{\Psi}^{N}[t]$ to the residual between the predicted $(\hat{\delta},\hat{E}_n)$ and the realized $(\delta,E_n)$.

% The training sub-twin $\widehat{\Omega}^{L}$ takes the split-learning variables $(l_n[t],\rho_n[t],\alpha_n[t])$ and the learning observation $o^{L}[t]$, and returns the predicted one-round loss decrease $\Delta\hat{\mathfrak{L}}[t]$ through a lightweight parametric regressor with parameters $\boldsymbol{\Psi}^{L}[t]$. Loop 2 fires at every federated-averaging instant and refits $\boldsymbol{\Psi}^{L}[t]$ on a sliding window of the realized $\{\Delta\mathfrak{L}[\tau]\}$ together with their corresponding split-learning inputs.

% The task sub-twin $\widehat{\Omega}^{T}$ returns the success-rate estimate $\hat{A}[t]$ in two modes. During planning it reads off the cached value parameterized by $\boldsymbol{\Psi}^{T}[t]$. During evaluation the current $\mathbf{W}[t]$ is rolled out on the LIBERO manipulation benchmark~\cite{Liu2023NeurIPS} to obtain the true $A[t]$ via Eq.~\eqref{eq:sys-A}, and Loop 3 refreshes $\boldsymbol{\Psi}^{T}[t]$ on the residual between $\hat{A}[t]$ and $A[t]$.
% A world model for the MDP is a predictive surrogate that, given state $s$ and candidate action $a$, returns $\hat{s}'$ and $\hat{r}$ without invoking the physical system. The cross-domain digital twin $\widehat{\Omega}[t]$ is this world model: the channel and learning sub-twins assemble the twin transition $\widehat{P}\triangleq\widehat{P}_l\circ\widehat{P}_w$, and the task sub-twin $\widehat{\Omega}^r$ supplies the predicted task-gain $\hat{r}^m[t]$.

% The three sub-twins each specialize to one layer of the stack. The channel sub-twin $\widehat{\Omega}^{w}$ takes the candidate allocation $(b_n,p_n)_{n=1}^{N}$ and the wireless observation $o^w[t]$, and returns the predicted maximum rate, round latency, and per-agent uplink energy $(\hat{R}^{U}_n[t],\hat{\ell}^{c}[t],\hat{E}^{U}_n[t])$ through Eqs.\eqref{eq:sys-Y}--\eqref{eq:sys-R}. Its parameters $\boldsymbol{\Psi}^w[t]$ are refined by the L1 loop.

% The learning-dynamics sub-twin $\widehat{\Omega}^{l}$ takes $(j_n,\rho_n,m_n)_{n=1}^{N}$ and returns the predicted aggregate loss decrease $\Delta\hat{L}[t]$. To preserve the architecture-specific gradient statistics of the foundation model, $\Delta\hat{L}[t]$ is produced by a shadow instance that runs one forward--backward pass on a held-aside minibatch under the candidate cut layers and compression ratios. The shadow instance is a separate copy of the production model that shares the production architecture but runs entirely on the server, so it incurs no wireless transmission cost. Its parameters $\boldsymbol{\Psi}^l[t]$ are refined by the L2 loop.

% The task sub-twin $\widehat{\Omega}^{r}$ supplies a per-round task-success estimate $\hat{A}[t]$ in two distinct modes. At planning time, $\widehat{\Omega}^{r}$ returns a cached estimate based on the latest L3-calibrated parameters $\boldsymbol{\Psi}^r[t]$, so that each CEM candidate is scored without invoking the simulator. At calibration time (every $E_{\mathrm{eval}}$ rounds), the current adapter $W[t]$ is rolled out in the LIBERO manipulation benchmark~\cite{Liu2023NeurIPS} to produce the true $A[t]$, which is then used by the L3 loop to refine $\boldsymbol{\Psi}^r[t]$ via Eq.\eqref{eq:sys-A}. The first mode is the cheap signal seen inside the inner CEM loop, while the second is expensive and runs on the slowest cadence.

% The intrinsic parameters $\boldsymbol{\Psi}[t]$ control how faithfully $\widehat{\Omega}[t]$ approximates $P$ and are never selected by the controller, whereas the action $a[t]$ is the per-round decision evaluated against the frozen $\boldsymbol{\Psi}[t]$. This separation makes the twin a planning instrument that evaluates candidate actions before execution, rather than merely a data generator for offline policy training.

\subsection{Decision-Making Process}
\label{sec:method-plan}

At each round $t$, TiLP picks the resource allocation $a^\star[t]$ by simulating $K$ rounds ahead inside $\widehat{\Omega}[t]$ for many candidate $K$-step action sequences and keeping the best one, where a learned actor $\pi_\theta(a\mid s)$ supplies the starting distribution for the candidates and a learned critic $Q_\phi(s,a)$ scores what would happen past the $K$-th simulated round. When the per-round compute budget cannot afford the simulation, $\pi_\theta(\cdot\mid s[t])$ alone is queried as a deployable fallback.

The search runs CEM on the mixed continuous-discrete action space. Each round, the CEM sampling distribution $\mu$ is initialized from $\pi_\theta(a\mid s[t])$. CEM then draws a population of $K$-step candidate sequences $\hat{a}[t],\dots,\hat{a}[t+K-1]$ from $\mu$, rolls each through $\widehat{\Omega}$ from $s[t]$ to predict the per-step rewards $\hat{r}[t+k]$ and the terminal state $\hat{s}[t+K]$, and assigns each candidate the score
\begin{equation}
  \hat{J} = \sum_{k=0}^{K-1}\gamma^{k}\,\hat{r}[t+k]+\gamma^{K}\,V(\hat{s}[t+K]),
  \label{eq:method-J}
\end{equation}
with the terminal value
\begin{equation}
  V(s) \triangleq \mathbb{E}_{a\sim\pi_\theta(\cdot\mid s)}\bigl[Q_\phi(s,a)\bigr].
  \label{eq:method-V}
\end{equation}
CEM then refits $\mu$ to the elite candidates by $\hat{J}$ and iterates. The horizon $K$ is kept small to bound the prediction error compounded through $\widehat{\Omega}$, and $\hat{a}^\star[t]$ is taken as the first action of the highest-$\hat{J}$ sequence.

The actor factorizes per-terminal,
\begin{equation}
  \pi_\theta(a\mid s)=\prod_{n=1}^{N}\pi_\theta(a_n\mid s),
  \label{eq:method-pi}
\end{equation}
For each terminal $n$, the continuous actions $(\mathrm{b}_n,\mathrm{p}_n,\rho_n)$ are sampled from a tanh-squashed Gaussian~\cite{Jennifer2018PMLR}, and the discrete actions $l_n$ and $\alpha_n$ from a Gumbel-softmax categorical~\cite{Eric2017ICLR} over $\mathcal{L}$ and a Bernoulli, respectively. The critic $Q_\phi(s,a)$ is a feed-forward network that maps the concatenated state-action vector to a scalar. Both networks are trained with SAC~\cite{Haarnoja2018ICML} on a mixed replay buffer of real transitions executed under $a^\star[t]$ and imaginary rollouts generated by $\pi_\theta$ through $\widehat{\Omega}$~\cite{Janner2019NeurIPS}.
% with each per-terminal factor $\pi_\theta(a_n\mid s)$ realized as tanh-squashed Gaussians on the continuous $(\mathrm{b}_n,\mathrm{p}_n,\rho_n)$, a Gumbel-softmax categorical over $\mathcal{L}$ on the cut layer $l_n$, and a Bernoulli on the schedule indicator $\alpha_n$. The critic $Q_\phi(s,a)$ is a feed-forward scalar head over the concatenated state-action vector. Both networks are trained by soft actor--critic (SAC)~\cite{Haarnoja2018ICML} on a mixed replay combining real FSL transitions executed under $a^\star[t]$ with imaginary trajectories rolled by $\pi_\theta$ through $\widehat{\Omega}$~\cite{Janner2019NeurIPS}.

This couples decision-making and learning into a single loop: $(\pi_\theta,Q_\phi)$ feed CEM's prior and terminal value, while CEM's executed $\hat{a}^\star[t]$ and the twin's imagined rollouts feed SAC's replay. Improvements in $(\pi_\theta,Q_\phi)$ tighten CEM's prior, and CEM's improved actions enrich the replay that trains $(\pi_\theta,Q_\phi)$.
% This couples planning and learning into a single loop: $(\pi_\theta,Q_\phi)$ feed CEM's prior and terminal value, while CEM's executed $a^\star[t]$ and the twin's imagined rollouts feed SAC's replay. Improvements in $(\pi_\theta,Q_\phi)$ tighten CEM's prior, and CEM's improved actions enrich the replay that trains $(\pi_\theta,Q_\phi)$.

% \subsection{Receding-Horizon Planning}
% \label{sec:method-plan}

% At each round $t$, TiLP selects the resource allocation $a^\star[t]$ by receding-horizon optimization over the composed twin. The planning horizon $K$ trades look-ahead quality against computational cost: a longer horizon accumulates prediction error from the twin, so $K$ is kept at a small integer in practice.

% The planner uses the cross-entropy method (CEM)~\cite{Rubinstein1999} on the mixed continuous-discrete action space. The CEM sampling distribution $\mu$ is seeded from the parametric actor $\pi_\theta(a\mid s)$, so that CEM begins from a warm-started prior rather than a uniform one. To stabilize finite-horizon planning, a terminal value is attached,
% \begin{equation}
%   V(s)\triangleq\mathbb{E}_{a\sim\pi_\theta(\cdot\mid s)}\bigl[Q_\phi(s,a)\bigr],
%   \label{eq:method-V}
% \end{equation}
% where $Q_\phi$ is the soft critic. Each candidate sequence is rolled $K$ steps through $\widehat{\Omega}$ and scored by a return estimate that sums the predicted per-step rewards and appends a terminal value to account for the rounds beyond the planning horizon,
% \begin{equation}
%   \hat{J}\!\bigl(a^{(i)}_{0:K-1}\bigr)
%   = \sum_{k=0}^{K-1}\gamma^{k}\hat{r}_k+\gamma^{K}V(\hat{s}_K).
%   \label{eq:method-J}
% \end{equation}
% The warm start from $\pi_\theta$ allows the planner to inherit the long-run policy improvement that receding-horizon search alone cannot capture.

% \subsection{Policy Training}
% \label{sec:method-sac}

% The actor $\pi_\theta$ and critic $Q_\phi$ are trained alongside the CEM planner: $\pi_\theta$ supplies the warm-start distribution $\mu$, and $Q_\phi$ supplies the terminal value $V(\hat{s}_K)$ in Eq.~\eqref{eq:method-J}. At deployment, the trained $\pi_\theta$ can be queried directly when the per-round compute budget does not permit CEM.

% Because the actor must handle continuous and discrete decision variables simultaneously, $\pi_\theta$ factorizes across action components: tanh-squashed Gaussians for the continuous variables $(b_n[t],p_n[t],\rho_n[t])$, a Gumbel-softmax categorical over $\mathcal{K}$ for the discrete cut layer $j_n[t]$, and a Bernoulli for the scheduling indicator $m_n[t]$. The critic $Q_\phi(s,a)$ takes the concatenated state and action vectors as input and outputs a scalar value estimate. Both networks are trained on a mixed replay $\mathcal{D}_b\!=\!\mathcal{D}_r\cup\mathcal{D}_v$, where $\mathcal{D}_r$ stores real FSL transitions $(s[t],a^\star[t],r[t],s[t+1])$ collected during execution and $\mathcal{D}_v$ holds $H$-step imaginary rollouts of $\pi_\theta$ through $\widehat{\Omega}$~\cite{Janner2019NeurIPS}. The rollout length $H$ is independent of the planning horizon $K$, since $\mathcal{D}_v$ feeds gradient updates rather than per-round decisions. The actor, critic, and a Polyak-averaged target critic are updated by the soft actor--critic (SAC) algorithm~\cite{Haarnoja2018ICML}, which maximizes the expected return plus an entropy bonus that encourages exploration.

\subsection{Algorithm and Multi-Scale Calibration}
\label{sec:method-proc}

Algorithm~\ref{alg:tilp} integrates the components above over $T$ rounds. Each round runs in three phases. Phase~I assembles the state and runs CEM through $\widehat{\Omega}$ to select $a^\star[t]$. Phase~II executes the FSL round under $a^\star[t]$ on the physical system and observes the realized cost. Phase~III updates the three sub-twins at three frequencies (every round, every $F$ rounds, and every $E_A$ rounds), each matching the time scale of the process it models. Each loop minimizes the prediction residual over its most recent observation window:
\begin{itemize}
  \item \textbf{Loop 1 (per round)} refines $\boldsymbol{\Psi}_1[t]$ on the residual between the predicted $(\hat{\delta},\hat{E}_n)$ and the realized $(\delta,E_n)$.
  \item \textbf{Loop 2 (per aggregation, every $F$ rounds)} refines $\boldsymbol{\Psi}_2[t]$ on the residual between the regressor-predicted $\Delta\hat{\mathfrak{L}}$ and the realized $\Delta\mathfrak{L}$ over the last $F$ rounds, immediately after the server-side update of Eq.~\eqref{eq:sys-upd-s}.
  \item \textbf{Loop 3 (per evaluation, every $E_{\mathrm{A}}$ rounds)} refines $\boldsymbol{\Psi}_3[t]$ on the residual between the cached $\hat{A}[t]$ and the realized $A[t]$ produced by a LIBERO rollout of $\mathbf{W}[t]$ via Eq.~\eqref{eq:sys-A}.
\end{itemize}
% The three cadences match the time scales of the three physical processes the sub-twins approximate, illustrated in~\ref{alg:tilp}. Together they keep $\widehat{\Omega}[t]$ informative for the BS throughout training.
% Algorithm~\ref{alg:tilp} integrates the components above over $R$ rounds. Each round runs in three phases. Phase~I assembles the state and runs CEM through $\widehat{\Omega}$ to select $a^\star[t]$. Phase~II executes the FSL round under $a^\star[t]$ on the physical system and observes the realized cost. Phase~III runs three calibration loops at three nested cadences. Each loop minimizes the prediction residual over its most recent observation window:
% \begin{itemize}
%   \item \textbf{L1 (per round)} refines $\boldsymbol{\Psi}^w[t]$ on the channel residual between the predicted $(\hat{\ell}^{c},\hat{E}^U_n)$ and the realized $(\ell^{c},E^U_n)$.
%   \item \textbf{L2 (per aggregation, every $F$ rounds)} refines $\boldsymbol{\Psi}^l[t]$ on the shadow-instance loss-trajectory residual over the last $F$ rounds, immediately after the federated average of Eq.~\eqref{eq:sys-fedavg}.
%   \item \textbf{L3 (per evaluation, every $E_{\mathrm{eval}}$ rounds)} refines $\boldsymbol{\Psi}^r[t]$ on the task-success residual produced by a LIBERO rollout of $W[t]$.
% \end{itemize}
% The three cadences match the time scales of the three physical processes the sub-twins approximate, illustrated in \cref{fig:twinloop}. Together they keep $\widehat{\Omega}[t]$ informative for receding-horizon planning throughout training.


\begin{algorithm}[t]
\small
\caption{TiLP: Twin-in-the-Loop Planner}
\label{alg:tilp}
\textbf{Input:} Initial model $\mathbf{W}[0]$; twin $\widehat{\Omega}[0]$ with sub-twin parameters $\boldsymbol{\Psi}_1[0],\boldsymbol{\Psi}_2[0],\boldsymbol{\Psi}_3[0]$; actor $\pi_\theta$, soft critic $Q_\phi$ with target $Q_{\phi^-}$; planning horizon $K$; aggregation interval $F$; evaluation interval $E_A$; CEM population $Y_1$, elites $Y_2$, iterations $I$; imagination rollout length $U$.
\begin{algorithmic}
  \STATE Initialize $\pi_\theta, Q_\phi$ randomly; empty the real and imagined replays
  \FOR{$t = 1, \ldots, T$}
    \colorbox{white}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\STATE \gray{$\triangleright$ \textit{Phase~I: Plan via CEM in $\widehat{\Omega}$}}}}
    \colorbox{rgb:red!2,65;green!30,60;blue!20,125}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\vbox{
      \STATE Assemble $s[t]$ per Eq.~\eqref{eq:method-state}; init $\mu\leftarrow\pi_\theta(\cdot\mid s[t])$
      \FOR{$i = 1, \ldots, I$}
        \STATE Draw $Y_1$ candidate $K$-step sequences from $\mu$; roll each through $\widehat{\Omega}$ and score by Eq.~\eqref{eq:method-J}
        \STATE Refit $\mu$ to the top-$Y_2$ elites
      \ENDFOR
      \STATE $a^\star[t]\leftarrow$ first action of the highest-$\hat{J}$ sequence
    }}}

    \colorbox{white}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\STATE \gray{$\triangleright$ \textit{Phase~II: Execute one FSL round}}}}
    \colorbox{rgb:red!2,65;green!30,90;blue!20,125}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\vbox{
      \STATE Broadcast $a^\star[t]$; each terminal with $\alpha_n[t]=1$ runs the client-side forward and backward passes per Eqs.~\eqref{eq:sys-Sfwd} and~\eqref{eq:sys-upd-c}; the server runs the server-side forward and backward passes per Eq.~\eqref{eq:sys-upd-s}
      \STATE Observe $\delta[t]$ and $\{E_n[t]\}_{n=1}^{N}$; compute $r[t]$ per Eqs.~\eqref{eq:method-reward} and~\eqref{eq:method-gamma}
    }}}

    \colorbox{white}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\STATE \gray{$\triangleright$ \textit{Phase~III: Multi-scale calibration}}}}
    \colorbox{rgb:red!60,100;green!20,90;blue!30,125}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\vbox{
      \STATE Loop 1: update $\boldsymbol{\Psi}_1[t]$ on the $(\hat{\delta}[t],\hat{E}_n[t])\!-\!(\delta[t],E_n[t])$ residual
      \STATE Append $(s[t],a^\star[t],r[t],s[t\!+\!1])$ to the real replay; roll a $U$-step imaginary trajectory under $\pi_\theta,\widehat{\Omega}$ into the imagined replay; SAC update on the union, soft-update $\phi^-$
      \IF{$t\bmod F = 0$}
        \STATE Federated-average $\{\mathbf{W}^{\textrm{C}}_n[t]\}_{n=1}^{N}$ using weights $|D_n|/D$; Loop 2: update $\boldsymbol{\Psi}_2[t]$ on the loss-reduction residual over the last $F$ rounds
      \ENDIF
      \IF{$t\bmod E_A = 0$}
        \STATE LIBERO rollout: $A[t]$ via Eq.~\eqref{eq:sys-A}; Loop 3: update $\boldsymbol{\Psi}_3[t]$ on the $\hat{A}[t]\!-\!A[t]$ residual
      \ENDIF
    }}}
  \ENDFOR
  \STATE \textbf{Output:} $\mathbf{W}[T]$, $A[T]$
\end{algorithmic}
\end{algorithm}

% The per-round planning cost amounts to $I\!\cdot\!Y_1\!\cdot\!K$ twin rollouts, with each step reducing to a closed-form evaluation in $\widehat{\Omega}^{N}$, one regressor forward pass in $\widehat{\Omega}^{L}$, and a cached lookup in $\widehat{\Omega}^{T}$, all well below one foundation-model forward--backward pass; among the three calibration loops, only the LIBERO rollout in Loop 3 is expensive.

% \begin{algorithm}[t]
% \small
% \caption{TiLP: Twin-in-the-Loop Planner}
% \label{alg:tilp}
% \textbf{Input:} Initial model $W[0]$; composed twin $\widehat{\Omega}$ with parameters $\boldsymbol{\Psi}[0]$; actor $\pi_\theta$, soft critic $Q_\phi$ with target $Q_{\phi^-}$; planning horizon $K$; aggregation interval $F$; evaluation interval $E_{\mathrm{eval}}$; CEM population $N_p$, elites $N_e$, iterations $I$; twin rollout length $H$.
% \begin{algorithmic}
%   \STATE Pre-calibrate $\boldsymbol{\Psi}[0]$; initialize $\pi_\theta, Q_\phi$ randomly; $\mathcal{D}_r,\mathcal{D}_v\!\leftarrow\!\varnothing$
%   \FOR{$t = 1, 2, \ldots, R$}
%     \colorbox{white}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\STATE \gray{$\triangleright$ \textit{Phase~I: State Assembly and Twin-Based Planning}}}}
%     \colorbox{rgb:red!2,65;green!30,60;blue!20,125}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\vbox{
%       \STATE Assemble $s[t]$ from channel state information (CSI), server logs, $\hat{A}[t\!-\!1]$, and $t/R$ per Eq.\eqref{eq:method-state}
%       \STATE Initialize CEM distribution $\mu$ from $\pi_\theta(\cdot\mid s[t])$ (warm start)
%       \FOR{$i = 1, \ldots, I$}
%         \STATE Sample $N_p$ candidate sequences $\{a^{(j)}_{0:K-1}\}_{j=1}^{N_p}$ from $\mu$
%         \FOR{each candidate $j$}
%           \STATE Roll $K$ steps through $\widehat{\Omega}$: channel sub-twin returns $(\hat{R}^{U}_n,\hat{\ell}^{c},\hat{E}^{U}_n)$, learning sub-twin returns $\Delta\hat{L}$, task sub-twin returns cached $\hat{A}$ from latest $\boldsymbol{\Psi}^r$; accumulate predicted reward $\hat{r}_k$
%           \STATE Compute $\hat{J}^{(j)}$ per Eq.\eqref{eq:method-J}
%         \ENDFOR
%         \STATE Retain top-$N_e$ elites by $\hat{J}$; refit $\mu$ to their empirical mean and variance
%       \ENDFOR
%       \STATE $a^\star[t] \leftarrow$ first action of the highest-$\hat{J}$ sequence
%     }}}

%     \colorbox{white}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\STATE \gray{$\triangleright$ \textit{Phase~II: FSL Round Execution}}}}
%     \colorbox{rgb:red!2,65;green!30,90;blue!20,125}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\vbox{
%       \STATE Broadcast $a^\star[t]$; form schedule $\mathcal{S}[t]\triangleq\{n:m_n[t]\!=\!1\}$
%       \FOR{each $n\in\mathcal{S}[t]$ \textbf{in parallel}}
%         \STATE Agent $n$: head forward pass (FP) $\to\mathbf{S}_n[t]$ per Eq.\eqref{eq:sys-Sfwd}; compress at $\rho_n[t]$; uplink over $(b_n[t],p_n[t])$
%         \STATE Server: tail FP on received batch, loss, tail backward pass (BP) $\to\mathbf{Z}_n[t]$; compress; downlink
%         \STATE Agent $n$: head BP with $\mathbf{Z}_n[t]$; update $W_{c,n}[t]$ per Eq.\eqref{eq:sys-upd-c}
%       \ENDFOR
%       \STATE Server updates tail adapter $W_s[t]$ per Eq.\eqref{eq:sys-upd-s}
%       \STATE Observe $\ell^{c}[t]$ and $\{E_n[t]\}_{n=1}^{N}$; compute $r[t]$ per Eqs.\eqref{eq:method-reward}--\eqref{eq:method-gamma}
%     }}}

%     \colorbox{white}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\STATE \gray{$\triangleright$ \textit{Phase~III: Multi-Scale Calibration}}}}
%     \colorbox{rgb:red!60,100;green!20,90;blue!30,125}{\parbox{\dimexpr\columnwidth-2\fboxsep-20pt\relax}{\vbox{
%       \STATE Update $\boldsymbol{\Psi}^w[t]$ via L1 loop (channel latency/energy residual)
%       \STATE Append $(s[t],a^\star[t],r[t],s[t\!+\!1])$ to $\mathcal{D}_r$
%       \STATE Generate $H$-step imaginary rollouts from $s[t]$ under $\pi_\theta$ and $\widehat{\Omega}$; append to $\mathcal{D}_v$
%       \STATE Update $\phi,\theta$ via actor--critic gradient steps on $\mathcal{D}_r\cup\mathcal{D}_v$; soft-update $\phi^-$
%       \IF{$(t+1)\bmod F = 0$}
%         \STATE Federated average per Eq.\eqref{eq:sys-fedavg}; broadcast $\overline{W}_c[t]$
%         \STATE Update $\boldsymbol{\Psi}^l[t]$ via L2 loop (loss-trajectory residual over last $F$ rounds)
%       \ENDIF
%       \IF{$t\bmod E_{\mathrm{eval}} = 0$}
%         \STATE Task rollout $\Rightarrow A[t]$; update $\boldsymbol{\Psi}^r[t]$ via L3 loop (task-success residual)
%       \ENDIF
%     }}}
%   \ENDFOR
%   \STATE \textbf{Output:} Trained model $W[R]$, task-success rate $A[R]$
% \end{algorithmic}
% \end{algorithm}

% The per-round planning cost is $I\!\cdot\!N_p\!\cdot\!K$ twin rollouts at $\mathcal{O}(c_w+c_l+c_r)$ per step, where $c_w$, $c_l$, and $c_r$ are the per-step costs of the channel, learning, and task sub-twins, dominated by the shadow forward--backward pass $c_l$. Phase~II costs one standard FSL round, and Phase~III amortizes calibration across the three cadences, with only the L3 rollout being expensive. The memory footprint is negligible relative to the foundation-model adapter storage.

